Region Growing Curriculum Generation for Reinforcement Learning

Learning a policy capable of moving an agent between any two states in the environment is important for many robotics problems involving navigation and manipulation. Due to the sparsity of rewards in such tasks, applying reinforcement learning in these scenarios can be challenging. Common approaches for tackling this problem include reward engineering with auxiliary rewards, requiring domain-specific knowledge or changing the objective. In this work, we introduce a method based on region-growing that allows learning in an environment with any pair of initial and goal states. Our algorithm first learns how to move between nearby states and then increases the difficulty of the start-goal transitions as the agent's performance improves. This approach creates an efficient curriculum for learning the objective behavior of reaching any goal from any initial state. In addition, we describe a method to adaptively adjust expansion of the growing region that allows automatic adjustment of the key exploration hyperparameter to environments with different requirements. We evaluate our approach on a set of simulated navigation and manipulation tasks, where we demonstrate that our algorithm can efficiently learn a policy in the presence of sparse rewards.

==> bibliorgraphy_fullnames.tex <==
%%% ====================================================================
%%%  BibTeX-file{
%%%     author          = "Gerry Murray",
%%%     version         = "1.2",
%%%     date            = "2 April 2012",
%%%     filename        = "acmsmall-sample-bibfile.bib",
%%%     address         = "ACM, NY",
%%%     email           = "murray at hq.acm.org",
%%%     codetable       = "ISO/ASCII",
%%%     keywords        = "ACM Reference Format, bibliography, citation, references",
%%%     supported       = "yes",
%%%     docstring       = "This BibTeX database file contains 'bibdata' entries
%%%                        that 'match' the examples provided in the Specifications Document
%%%                        AND, also, 'legacy'-type bibs. It should assist authors in 
%%%                        choosing the 'correct' at-bibtype and necessary bib-fields
%%%                        so as to obtain the appropriate ACM Reference Format output. 
%%%			   It also contains many 'Standard Abbreviations'. "
%%%  }
%%% ====================================================================

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }


% This file was created with JabRef 2.10.
% Encoding: UTF-8

% DRL

@misc{christiano17a,
Author = {Paul Christiano and Jan Leike and Tom B. Brown and Miljan Martic and Shane Legg and Dario Amodei},
Title = {Deep reinforcement learning from human preferences},
Year = {2017},
Eprint = {arXiv:1706.03741},
}


@inproceedings{duan16a,
  author    = {Yan Duan and
               Xi Chen and
               Rein Houthooft and
               John Schulman and
               Pieter Abbeel},
  title     = {Benchmarking Deep Reinforcement Learning for Continuous Control},
  booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
               {ICML} 2016, New York City, NY, USA},
  pages     = {1329--1338},
  year      = {2016},
  timestamp = {Tue, 12 Jul 2016 21:51:16 +0200},
}
%   url       = {http://jmlr.org/proceedings/papers/v48/duan16.html},

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- IRL


@inproceedings{schulmanTRPO,
  author    = {John Schulman and
               Sergey Levine and
               Pieter Abbeel and
               Michael I. Jordan and
               Philipp Moritz},
  title     = {Trust Region Policy Optimization},
  booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
               {ICML} 2015, Lille, France},
  pages     = {1889--1897},
  year      = {2015},
  timestamp = {Wed, 29 Mar 2017 16:45:25 +0200},
}
%   url       = {http://jmlr.org/proceedings/papers/v37/schulman15.html},

@article{schulmanGAE,
  author    = {John Schulman and
               Philipp Moritz and
               Sergey Levine and
               Michael I. Jordan and
               Pieter Abbeel},
  title     = {High-Dimensional Continuous Control Using Generalized Advantage Estimation},
  journal   = {CoRR},
  volume    = {abs/1506.02438},
  year      = {2015},
  timestamp = {Wed, 07 Jun 2017 14:41:00 +0200},
}
%   url       = {http://arxiv.org/abs/1506.02438},


@inproceedings{ng00irl,
  author    = {Andrew Y. Ng and
               Stuart J. Russell},
  title     = {Algorithms for Inverse Reinforcement Learning},
  booktitle = {Proceedings of the Seventeenth International Conference on Machine
               Learning {(ICML} 2000), Stanford University, Stanford, CA, USA},
  pages     = {663--670},
  year      = {2000},
  timestamp = {Sun, 21 Feb 2010 20:54:50 +0100},
}

@inproceedings{levine11irl,
  author    = {Sergey Levine and
               Zoran Popovic and
               Vladlen Koltun},
  title     = {Nonlinear Inverse Reinforcement Learning with Gaussian Processes},
  booktitle = {Advances in Neural Information Processing Systems 24: 25th Annual
               Conference on Neural Information Processing Systems 2011, Granada, Spain.},
  pages     = {19--27},
  year      = {2011},
  timestamp = {Thu, 11 Dec 2014 17:34:08 +0100},
}
%   url       = {http://papers.nips.cc/paper/4420-nonlinear-inverse-reinforcement-learning-with-gaussian-processes},

@inproceedings{abbeel04,
  author    = {Pieter Abbeel and
               Andrew Y. Ng},
  title     = {Apprenticeship learning via inverse reinforcement learning},
  booktitle = {Machine Learning, Proceedings of the Twenty-first International Conference
               {(ICML} 2004), Banff, Alberta, Canada},
  year      = {2004},
  timestamp = {Mon, 22 Oct 2007 13:54:01 +0200},
}
%   doi       = {10.1145/1015330.1015430},
%   url       = {http://doi.acm.org/10.1145/1015330.1015430},

% -- Init from demonstration

@conference{kalakrishnan12,
  author    = {Mrinal Kalakrishnan and
               Ludovic Righetti and
               Peter Pastor and
               Stefan Schaal},
  title     = {Learning Force Control Policies for Compliant Robotic Manipulation},
  booktitle = {Proceedings of the 29th International Conference on Machine Learning,
               {ICML} 2012, Edinburgh, Scotland, UK},
  year      = {2012},
  timestamp = {Wed, 29 Mar 2017 16:45:25 +0200},
}
%   url       = {http://icml.cc/2012/papers/642.pdf},


% --- Real robot RL

@article{popov17,
  added-at = {2017-05-02T00:00:00.000+0200},
  author = {Popov, Ivaylo and Heess, Nicolas and Lillicrap, Timothy P. and Hafner, Roland and Barth-Maron, Gabriel and Vecerik, Matej and Lampe, Thomas and Tassa, Yuval and Erez, Tom and Riedmiller, Martin A.},
  ee = {http://arxiv.org/abs/1704.03073},
  interhash = {fb9445cf1161dd52850c5f28a93cf440},
  intrahash = {7a107f3ad1a1db9f9c08456c1a327ca8},
  journal = {CoRR},
  keywords = {dblp},
  timestamp = {2017-05-03T11:36:13.000+0200},
  title = {Data-efficient Deep Reinforcement Learning for Dexterous Manipulation.},
  volume = {abs/1704.03073},
  year = 2017
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1704.html#PopovHLHBVLTER17},



% --- Classics

@misc{mnih2013playing,
  added-at = {2014-12-14T17:55:47.000+0100},
  author = {Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
  description = {Playing Atari with Deep Reinforcement Learning},
  interhash = {78966703f649bae69a08a6a23a4e8879},
  intrahash = {f4760edc252cd402821a341bda0026bf},
  keywords = {arxiv cs},
  timestamp = {2014-12-14T17:55:47.000+0100},
  title = {Playing Atari with Deep Reinforcement Learning},
  year = 2013
}
%   note = {cite arxiv:1312.5602Comment: NIPS Deep Learning Workshop 2013},
%   url = {http://arxiv.org/abs/1312.5602},
%   abstract = {We present the first deep learning model to successfully learn control
% policies directly from high-dimensional sensory input using reinforcement
% learning. The model is a convolutional neural network, trained with a variant
% of Q-learning, whose input is raw pixels and whose output is a value function
% estimating future rewards. We apply our method to seven Atari 2600 games from
% the Arcade Learning Environment, with no adjustment of the architecture or
% learning algorithm. We find that it outperforms all previous approaches on six
% of the games and surpasses a human expert on three of them.},


@article{guo16,
  added-at = {2016-05-02T00:00:00.000+0200},
  author = {Guo, Xiaoxiao and Singh, Satinder P. and Lewis, Richard L. and Lee, Honglak},
  ee = {http://arxiv.org/abs/1604.07095},
  interhash = {be3de07d03eb4fcc634babe3f776f7a4},
  intrahash = {cbe3703257d6014d4d1476519c43e2b0},
  journal = {CoRR},
  keywords = {dblp},
  timestamp = {2016-05-03T11:42:02.000+0200},
  title = {Deep Learning for Reward Design to Improve Monte Carlo Tree Search in ATARI Games.},
  volume = {abs/1604.07095},
  year = 2016
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1604.html#GuoSLL16},


@article{silver16alphago,
  author    = {David Silver and
               Aja Huang and
               Chris J. Maddison and
               Arthur Guez and
               Laurent Sifre and
               George van den Driessche and
               Julian Schrittwieser and
               Ioannis Antonoglou and
               Vedavyas Panneershelvam and
               Marc Lanctot and
               Sander Dieleman and
               Dominik Grewe and
               John Nham and
               Nal Kalchbrenner and
               Ilya Sutskever and
               Timothy P. Lillicrap and
               Madeleine Leach and
               Koray Kavukcuoglu and
               Thore Graepel and
               Demis Hassabis},
  title     = {Mastering the game of Go with deep neural networks and tree search},
  journal   = {Nature},
  volume    = {529},
  number    = {7587},
  pages     = {484--489},
  year      = {2016},
  timestamp = {Sat, 20 May 2017 00:24:51 +0200},
}
%   url       = {https://doi.org/10.1038/nature16961},
%   doi       = {10.1038/nature16961},


@article{goodfellow14,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
}
% url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}

% --- GPS

@article{levine15,
  added-at = {2015-02-02T00:00:00.000+0100},
  author = {Levine, Sergey and Wagener, Nolan and Abbeel, Pieter},
  ee = {http://arxiv.org/abs/1501.05611},
  interhash = {f56875b1dbd0b2b12f7e1c45bd05884e},
  intrahash = {58e856f9a3fafd7488ac88134c5c2030},
  journal = {CoRR},
  keywords = {dblp},
  timestamp = {2015-06-18T04:19:12.000+0200},
  title = {Learning Contact-Rich Manipulation Skills with Guided Policy Search.},
  volume = {abs/1501.05611},
  year = 2015
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1501.html#LevineWA15},

@inproceedings{finn16,
  author    = {Chelsea Finn and
               Sergey Levine and
               Pieter Abbeel},
  title     = {Guided Cost Learning: Deep Inverse Optimal Control via Policy Optimization},
  booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
               {ICML} 2016, New York City, NY, USA},
  pages     = {49--58},
  year      = {2016},
  timestamp = {Tue, 12 Jul 2016 21:51:16 +0200},
}

@article{chebotar16b,
  author = {Chebotar, Yevgen and Kalakrishnan, Mrinal and Yahya, Ali and Li, Adrian and Schaal, Stefan and Levine, Sergey},
  ee = {http://arxiv.org/abs/1610.00529},
  journal = {CoRR},
  keywords = {dblp},
  timestamp = {2016-11-03T11:35:13.000+0100},
  title = {Path Integral Guided Policy Search.},
  volume = {abs/1610.00529},
  year = 2016
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1610.html#ChebotarKYLSL16},

@article{chebotar17a,
  author    = {Yevgen Chebotar and
               Karol Hausman and
               Marvin Zhang and
               Gaurav S. Sukhatme and
               Stefan Schaal and
               Sergey Levine},
  title     = {Combining Model-Based and Model-Free Updates for Trajectory-Centric
               Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1703.03078},
  year      = {2017},
  timestamp = {Wed, 07 Jun 2017 14:42:40 +0200}
}
%   url       = {http://arxiv.org/abs/1703.03078},

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- Automatic curriculum

@Article{Sukhbaatar17,
Author = {Sainbayar Sukhbaatar and Zeming Lin and Ilya Kostrikov and Gabriel Synnaeve and Arthur Szlam},
Title = {Intrinsic Motivation and Automatic Curricula via Asymmetric Self-Play},
Year = {2017},
Eprint = {arXiv:1703.05407},
}

@Article{Held17,
Author = {David Held and Xinyang Geng and Carlos Florensa and Pieter Abbeel},
Title = {Automatic Goal Generation for Reinforcement Learning Agents},
Year = {2017},
Eprint = {arXiv:1705.06366},
}

@article{florensa17a,
  author    = {Carlos Florensa and
               David Held and
               Markus Wulfmeier and
               Pieter Abbeel},
  title     = {Reverse Curriculum Generation for Reinforcement Learning},
  journal   = {CoRR},
  volume    = {abs/1707.05300},
  year      = {2017},
  timestamp = {Sat, 05 Aug 2017 14:56:18 +0200},
}
%   url       = {http://arxiv.org/abs/1707.05300},

@article{matiisen17,
Author = {Tambet Matiisen and Avital Oliver and Taco Cohen and John Schulman},
Title = {Teacher-Student Curriculum Learning},
Year = {2017},
Eprint = {arXiv:1707.00183},
}


@inproceedings{svetlik17,
  author    = {Maxwell Svetlik and
               Matteo Leonetti and
               Jivko Sinapov and
               Rishi Shah and
               Nick Walker and
               Peter Stone},
  title     = {Automatic Curriculum Graph Generation for Reinforcement Learning Agents},
  booktitle = {Proceedings of the Thirty-First {AAAI} Conference on Artificial Intelligence,
               San Francisco, California, USA},
  pages     = {2590--2596},
  year      = {2017},
  timestamp = {Mon, 06 Mar 2017 11:36:24 +0100},
}
%   url       = {http://aaai.org/ocs/index.php/AAAI/AAAI17/paper/view/14961},

@article{forestier17,
  author    = {S{\'{e}}bastien Forestier and
               Yoan Mollard and
               Pierre{-}Yves Oudeyer},
  title     = {Intrinsically Motivated Goal Exploration Processes with Automatic
               Curriculum Learning},
  journal   = {CoRR},
  volume    = {abs/1708.02190},
  year      = {2017},
  timestamp = {Tue, 05 Sep 2017 10:03:46 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1708-02190},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
%   url       = {http://arxiv.org/abs/1708.02190},


@misc{sharma17a,
Author = {Sahil Sharma and Ashutosh Jha and Parikshit Hegde and Balaraman Ravindran},
Title = {Learning to Multi-Task by Active Sampling},
Year = {2017},
Eprint = {arXiv:1702.06053},
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% --- Curriculum


@article{zaremba14,
  author    = {Wojciech Zaremba and
               Ilya Sutskever},
  title     = {Learning to Execute},
  journal   = {CoRR},
  volume    = {abs/1410.4615},
  year      = {2014},
  timestamp = {Wed, 07 Jun 2017 14:41:29 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/ZarembaS14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
%   url       = {http://arxiv.org/abs/1410.4615},

@inproceedings{bengio15a,
  author    = {Samy Bengio and
               Oriol Vinyals and
               Navdeep Jaitly and
               Noam Shazeer},
  title     = {Scheduled Sampling for Sequence Prediction with Recurrent Neural Networks},
  booktitle = {Advances in Neural Information Processing Systems 28: Annual Conference
               on Neural Information Processing Systems 2015, December 7-12, 2015,
               Montreal, Quebec, Canada},
  pages     = {1171--1179},
  year      = {2015},
  timestamp = {Fri, 08 Apr 2016 19:32:53 +0200},
}
%   url       = {http://papers.nips.cc/paper/5956-scheduled-sampling-for-sequence-prediction-with-recurrent-neural-networks},

@inproceedings{wu17a,
author = {Yuxin Wu and Yuandong Tian},
title = {Training agent for first-person shooter game with actor-critic curriculum learning},
booktitle = {International Conference on Learning Representations (ICLR)},
Year = {2017},
}

@article{hees17,
  author    = {Nicolas Heess and
               Dhruva TB and
               Srinivasan Sriram and
               Jay Lemmon and
               Josh Merel and
               Greg Wayne and
               Yuval Tassa and
               Tom Erez and
               Ziyu Wang and
               S. M. Ali Eslami and
               Martin A. Riedmiller and
               David Silver},
  title     = {Emergence of Locomotion Behaviours in Rich Environments},
  journal   = {CoRR},
  volume    = {abs/1707.02286},
  year      = {2017},
  timestamp = {Tue, 08 Aug 2017 15:06:57 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/HeessTSLMWTEWER17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
%   url       = {http://arxiv.org/abs/1707.02286},


% --- Hierarchical RL

@article{bacon_corr16,
  author = {Bacon, Pierre-Luc and Harb, Jean and Precup, Doina},
  ee = {http://arxiv.org/abs/1609.05140},
  interhash = {1228758ed5ccc479d462cd4472d7a483},
  intrahash = {e3f0e039960a7c24e757f3f86933e824},
  journal = {CoRR},
  keywords = {dblp},
  timestamp = {2016-10-04T11:33:44.000+0200},
  title = {The Option-Critic Architecture.},
  volume = {abs/1609.05140},
  year = 2016
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1609.html#BaconHP16},

@inproceedings{mankowitz__nips16,
  author = {Mankowitz, Daniel J. and Mann, Timothy Arthur and Mannor, Shie},
  booktitle = {NIPS},
  editor = {Lee, Daniel D. and Sugiyama, Masashi and Luxburg, Ulrike V. and Guyon, Isabelle and Garnett, Roman},
  ee = {http://papers.nips.cc/paper/6350-adaptive-skills-adaptive-partitions-asap},
  interhash = {544f6de0d585c9e71af301e461204fb7},
  intrahash = {9b09b8ad0e49ee8acbe5cf556791d67b},
  keywords = {dblp},
  pages = {1588-1596},
  timestamp = {2016-12-17T11:33:40.000+0100},
  title = {Adaptive Skills Adaptive Partitions (ASAP).},
  year = 2016
}
%   url = {http://dblp.uni-trier.de/db/conf/nips/nips2016.html#MankowitzMM16},


@inproceedings{vashnevets17,
  title={},
  author={Petrovskaya, Anna and Park, Jaeheung and Khatib, Oussama},
  booktitle={Proceedings 2017 International Conference on Robotics and Automation},
  pages={568--573},
  year={2007},
  organization={IEEE}
}

@article{pinto16,
    author = {Pinto, L},
    title = {{The Curious Robot: Learning Visual Representations via Physical Interactions}},
    journal = {Arxiv preprint hep-th},
    year = {2016}
}
% url = {https://arxiv.org/pdf/1604.01360v2.pdf}

@article{denil16,
  author = {Denil, Misha and Agrawal, Pulkit and Kulkarni, Tejas D. and Erez, Tom and Battaglia, Peter and de Freitas, Nando},
  ee = {http://arxiv.org/abs/1611.01843},
  interhash = {35b457681fe375d619abd2c4fc145933},
  intrahash = {9018936cec18c9e3659bf5f1607a291b},
  journal = {CoRR},
  keywords = {dblp},
  title = {Learning to Perform Physics Experiments via Deep Reinforcement Learning.},
  volume = {abs/1611.01843},
  year = 2016
}
%   url = {http://dblp.uni-trier.de/db/journals/corr/corr1611.html#DenilAKEBF16}

@inproceedings{kulkarni16a,
  author    = {Tejas D. Kulkarni and
               Karthik Narasimhan and
               Ardavan Saeedi and
               Josh Tenenbaum},
  title     = {Hierarchical Deep Reinforcement Learning: Integrating Temporal Abstraction
               and Intrinsic Motivation},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {3675--3683},
  year      = {2016},
  timestamp = {Fri, 03 Mar 2017 14:59:41 +0100},
}
  %   url       = {http://papers.nips.cc/paper/6233-hierarchical-deep-reinforcement-learning-integrating-temporal-abstraction-and-intrinsic-motivation}


@article{mechado16a,
  author    = {Marlos C. Machado and
               Michael H. Bowling},
  title     = {Learning Purposeful Behaviour in the Absence of Rewards},
  journal   = {CoRR},
  volume    = {abs/1605.07700},
  year      = {2016},
  timestamp = {Wed, 01 Jun 2016 15:51:07 +0200},
}
%   url       = {http://arxiv.org/abs/1605.07700}



@inproceedings{houthooft_nips16,
  author    = {Rein Houthooft and
               Xi Chen and
               Xi Chen and
               Yan Duan and
               John Schulman and
               Filip De Turck and
               Pieter Abbeel},
  title     = {{VIME:} Variational Information Maximizing Exploration},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {1109--1117},
  year      = {2016},
  timestamp = {Fri, 03 Mar 2017 14:59:41 +0100},
}
%   url       = {http://papers.nips.cc/paper/6591-vime-variational-information-maximizing-exploration}


@inproceedings{mohamed_nips15,
  author = {Mohamed, Shakir and Rezende, Danilo Jimenez},
  booktitle = {NIPS},
  editor = {Cortes, Corinna and Lawrence, Neil D. and Lee, Daniel D. and Sugiyama, Masashi and Garnett, Roman},
  ee = {http://papers.nips.cc/paper/5668-variational-information-maximisation-for-intrinsically-motivated-reinforcement-learning},
  interhash = {f63c536d0d44e0296a52388226ac8f1e},
  intrahash = {029e459e7b66405753cb0944ec8be90a},
  keywords = {dblp},
  pages = {2125-2133},
  timestamp = {2016-04-09T11:42:47.000+0200},
  title = {Variational Information Maximisation for Intrinsically Motivated Reinforcement Learning.},
  year = 2015
}
%   url = {http://dblp.uni-trier.de/db/conf/nips/nips2015.html#MohamedR15},


@article{agrawal_corr16,
  author    = {Pulkit Agrawal and
               Ashvin Nair and
               Pieter Abbeel and
               Jitendra Malik and
               Sergey Levine},
  title     = {Learning to Poke by Poking: Experiential Learning of Intuitive Physics},
  journal   = {CoRR},
  volume    = {abs/1606.07419},
  year      = {2016},
  timestamp = {Fri, 01 Jul 2016 17:39:49 +0200},
}
%   url       = {http://arxiv.org/abs/1606.07419}


@inproceedings{sun11,
  author    = {Yi Sun and
               Faustino J. Gomez and
               J{\"{u}}rgen Schmidhuber},
  title     = {Planning to Be Surprised: Optimal Bayesian Exploration in Dynamic
               Environments},
  booktitle = {Artificial General Intelligence - 4th International Conference, {AGI}
               2011, Mountain View, CA, USA, August 3-6, 2011. Proceedings},
  pages     = {41--51},
  year      = {2011},
  doi       = {10.1007/978-3-642-22887-2_5},
  timestamp = {Thu, 04 Aug 2011 08:38:04 +0200},
}
% url       = {http://dx.doi.org/10.1007/978-3-642-22887-2_5},




% ---- Intrinsic motivation

@article{jaderberg16,
  author    = {Max Jaderberg and
               Volodymyr Mnih and
               Wojciech Marian Czarnecki and
               Tom Schaul and
               Joel Z. Leibo and
               David Silver and
               Koray Kavukcuoglu},
  title     = {Reinforcement Learning with Unsupervised Auxiliary Tasks},
  journal   = {CoRR},
  volume    = {abs/1611.05397},
  year      = {2016},
  timestamp = {Wed, 07 Jun 2017 14:40:03 +0200},
}
%   url       = {http://arxiv.org/abs/1611.05397},

@inproceedings{houthooft16,
  author    = {Rein Houthooft and
               Xi Chen and
               Xi Chen and
               Yan Duan and
               John Schulman and
               Filip De Turck and
               Pieter Abbeel},
  title     = {{VIME:} Variational Information Maximizing Exploration},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {1109--1117},
  year      = {2016},
  timestamp = {Fri, 03 Mar 2017 14:59:41 +0100}
}

@article{schossau16,
  author    = {Jory Schossau and
               Christoph Adami and
               Arend Hintze},
  title     = {Information-Theoretic Neuro-Correlates Boost Evolution of Cognitive
               Systems},
  journal   = {Entropy},
  volume    = {18},
  number    = {1},
  pages     = {6},
  year      = {2016},
  doi       = {10.3390/e18010006},
  timestamp = {Wed, 14 Jun 2017 20:33:03 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/entropy/SchossauAH16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
%   url       = {https://doi.org/10.3390/e18010006},

@inproceedings{subramanian16,
  author    = {Kaushik Subramanian and
               Charles Lee Isbell Jr. and
               Andrea Lockerd Thomaz},
  title     = {Exploration from Demonstration for Interactive Reinforcement Learning},
  booktitle = {Proceedings of the 2016 International Conference on Autonomous Agents
               {\&} Multiagent Systems, Singapore},
  pages     = {447--456},
  year      = {2016},
  timestamp = {Fri, 20 May 2016 21:03:38 +0200},
}
%   url       = {http://dl.acm.org/citation.cfm?id=2936990},

@inproceedings{lopes12,
  author    = {Manuel Lopes and
               Tobias Lang and
               Marc Toussaint and
               Pierre{-}Yves Oudeyer},
  title     = {Exploration in Model-based Reinforcement Learning by Empirically Estimating
               Learning Progress},
  booktitle = {Advances in Neural Information Processing Systems 25: 26th Annual
               Conference on Neural Information Processing Systems 2012, Lake Tahoe, Nevada, United States.},
  pages     = {206--214},
  year      = {2012},
  timestamp = {Mon, 15 Dec 2014 13:33:40 +0100},
}

@article{stadie15,
  author    = {Bradly C. Stadie and
               Sergey Levine and
               Pieter Abbeel},
  title     = {Incentivizing Exploration In Reinforcement Learning With Deep Predictive
               Models},
  journal   = {CoRR},
  volume    = {abs/1507.00814},
  year      = {2015},
  timestamp = {Wed, 07 Jun 2017 14:40:03 +0200},
}
%   url       = {http://arxiv.org/abs/1507.00814},

@article{oudeyer07,
  author    = {Pierre{-}Yves Oudeyer and
               Fr{\'{e}}d{\'{e}}ric Kaplan and
               Verena Vanessa Hafner},
  title     = {Intrinsic Motivation Systems for Autonomous Mental Development},
  journal   = {{IEEE} Trans. Evolutionary Computation},
  volume    = {11},
  number    = {2},
  pages     = {265--286},
  year      = {2007},
  doi       = {10.1109/TEVC.2006.890271},
  timestamp = {Thu, 08 Jun 2017 09:05:42 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/tec/OudeyerKH07},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}
%   url       = {https://doi.org/10.1109/TEVC.2006.890271},

@article{schmidhuber10,
  author    = {J{\"{u}}rgen Schmidhuber},
  title     = {Formal Theory of Creativity, Fun, and Intrinsic Motivation {(1990-2010)}},
  journal   = {{IEEE} Trans. Autonomous Mental Development},
  volume    = {2},
  number    = {3},
  pages     = {230--247},
  year      = {2010},
  doi       = {10.1109/TAMD.2010.2056368},
  timestamp = {Sat, 27 May 2017 14:23:02 +0200}
}
%   url       = {https://doi.org/10.1109/TAMD.2010.2056368},

@inproceedings{bellemare16a,
  author    = {Marc G. Bellemare and
               Sriram Srinivasan and
               Georg Ostrovski and
               Tom Schaul and
               David Saxton and
               R{\'{e}}mi Munos},
  title     = {Unifying Count-Based Exploration and Intrinsic Motivation},
  booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
               on Neural Information Processing Systems 2016, December 5-10, 2016,
               Barcelona, Spain},
  pages     = {1471--1479},
  year      = {2016},
  url       = {http://papers.nips.cc/paper/6383-unifying-count-based-exploration-and-intrinsic-motivation},
  timestamp = {Fri, 03 Mar 2017 14:59:41 +0100},
}

@inproceedings{ostrovski17a,
  author    = {Georg Ostrovski and
               Marc G. Bellemare and
               A{\"{a}}ron van den Oord and
               R{\'{e}}mi Munos},
  title     = {Count-Based Exploration with Neural Density Models},
  booktitle = {Proceedings of the 34th International Conference on Machine Learning,
               {ICML} 2017, Sydney, NSW, Australia},
  pages     = {2721--2730},
  year      = {2017},
  timestamp = {Wed, 16 Aug 2017 11:08:55 +0200},
}
%   url       = {http://proceedings.mlr.press/v70/ostrovski17a.html},

@inproceedings{martin17,
  author    = {Jarryd Martin and
               Suraj Narayanan Sasikumar and
               Tom Everitt and
               Marcus Hutter},
  title     = {Count-Based Exploration in Feature Space for Reinforcement Learning},
  booktitle = {Proceedings of the Twenty-Sixth International Joint Conference on
               Artificial Intelligence, {IJCAI} 2017, Melbourne, Australia},
  pages     = {2471--2478},
  year      = {2017},
  doi       = {10.24963/ijcai.2017/344},
  timestamp = {Tue, 15 Aug 2017 14:48:05 +0200},
}
%   url       = {https://doi.org/10.24963/ijcai.2017/344},

% ---- Tactile: point of contact

@inproceedings{petrovskaya07,
  title={Probabilistic estimation of whole body contacts for multi-contact robot control},
  author={Petrovskaya, Anna and Park, Jaeheung and Khatib, Oussama},
  booktitle={Proceedings 2007 IEEE International Conference on Robotics and Automation},
  pages={568--573},
  year={2007},
  organization={IEEE}
}



@inproceedings{bruyninckx95,
  title={Peg-on-hole: a model based solution to peg and hole alignment},
  author={Bruyninckx, Herman and Dutre, Stefan and De Schutter, Joris},
  booktitle={Robotics and Automation, 1995. Proceedings., 1995 IEEE International Conference on},
  volume={2},
  pages={1919--1924},
  year={1995},
  organization={IEEE}
}

@inproceedings{felip14,
  title={Multi-sensor and prediction fusion for contact detection and localization},
  author={Felip, Javier and Morales, Antonio and Asfour, Tamim},
  booktitle={2014 IEEE-RAS Int. Conf. on Humanoid Robots},
  pages={601--607},
  year={2014},
  organization={IEEE}
}

@article{huber94,
  author = {Huber, Manfred and Grupen, Roderic A.},
  ee = {http://dx.doi.org/10.1109/70.285582},
  interhash = {8a9464ea81405a79ba289673ca7a762f},
  intrahash = {d45ddddf2e7c174ed0316134eb6bae28},
  journal = {IEEE T. Robotics and Automation},
  keywords = {dblp},
  number = 1,
  pages = {23-33},
  timestamp = {2014-01-16T11:34:07.000+0100},
  title = {2-D contact detection and localization using proprioceptive information.},
  volume = 10,
  year = 1994
}
%   url = {http://dblp.uni-trier.de/db/journals/trob/trob10.html#HuberG94},

@phdthesis{haidacher04,
    title    = {Contact Point and Object Position from Force/Torque and Position Sensors for Grasps with a Dextrous Robotic Hand},
    school   = {Technical University of Munich},
    author   = {Haidacher, Steffen},
    year     = {2004}, 
}
    % url      = {http://mediatum.ub.tum.de/doc/601587/601587.pdf},

@inproceedings{koonjul11,
  title={Measuring contact points from displacements with a compliant, articulated robot hand},
  author={Koonjul, Gurdayal S and Zeglin, Garth J and Pollard, Nancy S},
  booktitle={Robotics and Automation (ICRA), 2011 IEEE International Conference on},
  pages={489--495},
  year={2011},
  organization={IEEE}
}

@article{cucco14,
  author = {D’Ippolito, Filippo  and Alonge, Francesco  and Cucco, Elisa },
  journal = {Int J. Advanced Robotic Systems},
  title = {Contact Estimation in Robot Interaction},
  year = 2014
}
%   url = {http://cdn.intechopen.com/pdfs-wm/47180.pdf},

@article{likar14,
  title={External Joint Torque-based Estimation of Contact Information},
  author={Likar, Nejc and Zlajpah, Leon},
  journal={International Journal of Advanced Robotic Systems},
  volume={11},
  year={2014},
  publisher={InTech}  
}



@inproceedings{bernabe13,
  title={Contact localization through robot and object motion from point clouds},
  author={Bernab{\'e}, Jos{\'e} A and Felip, Javier and Del Pobil, Angel P and Morales, Antonio},
  booktitle={2013 13th IEEE-RAS International Conference on Humanoid Robots (Humanoids)},
  pages={268--273},
  year={2013},
  organization={IEEE}
}

@article{allen99,
  author = {Allen, Peter K. and Miller, Andrew T. and Oh, Paul Y. and Leibowitz, Brian S.},
  description = {MAPS citations},
  interhash = {29cbeaaea8ae8bf42e085bc330b6367b},
  intrahash = {be8c05631f6a0c4f67c0b0feb81a2379},
  journal = {Int. J. Intelligent Machines},
  keywords = {imported recognition},
  pages = {129--149},
  timestamp = {2009-06-09T23:55:27.000+0200},
  title = {Integration of vision, force and tactile sensing for grasping},
  year = 1999
}



@inproceedings{eppner15,
  author = {Eppner, Clemens and Brock, Oliver},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2015.7139886},
  interhash = {0f15488ad4268e36855c4026ba5da230},
  intrahash = {ab5e88a1f8c2e668d4c777b267e4ecbd},
  isbn = {978-1-4799-6923-4},
  keywords = {dblp},
  pages = {4947-4952},
  publisher = {IEEE},
  timestamp = {2015-07-14T11:39:49.000+0200},
  title = {Planning grasp strategies That Exploit Environmental Constraints.},
  year = 2015
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2015.html#EppnerB15},



@inproceedings{ishikawa96,
  title={Estimation of contact position between a grasped object and the environment based on sensor fusion of vision and force},
  author={Ishikawa, Tornohiko and Sakane, Shigeyuki and Sato, Tomomasa and Tsukune, Hideo},
  booktitle={Multisensor Fusion and Integration for Intelligent Systems, 1996. IEEE/SICE/RSJ International Conference on},
  pages={116--123},
  year={1996},
  organization={IEEE}
}

@inproceedings{tully12,
  author = {Tully, Stephen and Bajo, Andrea and Kantor, George and Choset, Howie and Simaan, Nabil},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2012.6225080},
  interhash = {7c16da2f47e76afd00f8a9a61d147605},
  intrahash = {8c8b47ad89dd4beab3d879321f7879fc},
  isbn = {978-1-4673-1403-9},
  keywords = {dblp},
  pages = {3388-3394},
  publisher = {IEEE},
  timestamp = {2012-07-20T11:35:14.000+0200},
  title = {Constrained filtering with contact detection data for the localization and registration of continuum robots in flexible environments.},
  year = 2012
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2012.html#TullyBKCS12},


@inproceedings{hovland97,
  title={Combining force and position measurements for the monitoring of robotic assembly},
  author={Hovland, Geir E and McCarragher, Brenan J},
  booktitle={Intelligent Robots and Systems, 1997. IROS'97., Proceedings of the 1997 IEEE/RSJ Int. Conf. on},
  volume={2},
  pages={654--660},
  year={1997},
  organization={IEEE}
}

@article{yang02,
  author = {Yang, Guilin and Chen, I-Ming and Yeo, Song Huat and Lim, Wee Kiat},
  date = {2009-06-29},
  description = {dblp},
  ee = {http://dx.doi.org/10.1017/S0263574702004101},
  interhash = {a89326a46d5f1667421e1f310bff3e81},
  intrahash = {1f0b1cd5a9ff17d58f2dcfb7a61b063a},
  journal = {Robotica},
  keywords = {dblp},
  number = 4,
  pages = {367-374},
  timestamp = {2009-07-16T14:47:34.000+0200},
  title = {Simultaneous base and tool calibration for self-calibrated parallel robots.},
  volume = 20,
  year = 2002
}
%   url = {http://dblp.uni-trier.de/db/journals/robotica/robotica20.html#YangCYL02},

@article{cheah06,
  author = {Cheah, Chien-Chern and Chao Liu and Slotine, Jean-Jacques E.},
  ee = {http://dx.doi.org/10.1109/TAC.2006.876943},
  interhash = {0366abe9fbc8012b57ea2d6efab1ca14},
  intrahash = {c2528171e3495f8975495b3d98dcdc8d},
  journal = {IEEE Trans. Automat. Contr.},
  keywords = {dblp},
  number = 6,
  pages = {1024-1029},
  timestamp = {2012-10-12T11:33:09.000+0200},
  title = {Adaptive Jacobian tracking control of robots with uncertainties in kinematic, dynamic and actuator models.},
  volume = 51,
  year = 2006
}
%   url = {http://dblp.uni-trier.de/db/journals/tac/tac51.html#Cheah0S06},

@inproceedings{muto94,
  author = {yo Muto, Shin and ichiro Shimokura, Ken},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ROBOT.1994.351408},
  interhash = {508e255fa9665ac52dbdbc510c76a078},
  intrahash = {757d18913a672a6e3e9514bd77b8f3b1},
  isbn = {0-8186-5330-2},
  keywords = {dblp},
  pages = {674-681},
  publisher = {IEEE Computer Society},
  timestamp = {2013-02-21T11:43:52.000+0100},
  title = {Teaching and Control of Robot Contour-Tracking Using Contact Point Detection.},
  year = 1994
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra1994-1.html#MutoS94},

@inproceedings{madry2014ICRA,
  author={Marianna Madry and Liefeng Bo and Danica Kragic and Dieter Fox}, 
  booktitle={IEEE International Conference on Robotics and Automation (ICRA)}, 
  title={{ST-HMP: Unsupervised Spatio-Temporal Feature Learning for Tactile Data}}, 
  year={2014}, 
  month={may}, 
}

@inproceedings{luo15,
  author = {Luo, Shan and Mou, Wenxuan and Althoefer, Kaspar and Liu, Hongbin},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2015.7139743},
  interhash = {7e23401d4721711b09d2de880cdacd83},
  intrahash = {bee5b6e9637e9c893e26c0bea20c218d},
  isbn = {978-1-4799-6923-4},
  keywords = {dblp},
  pages = {3903-3908},
  publisher = {IEEE},
  timestamp = {2015-07-14T11:39:49.000+0200},
  title = {Localizing the object contact through matching tactile features with visual map.},
  year = 2015
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2015.html#LuoMAL15},

@inproceedings{Hu00,
  title={Visual cues for imminent object contact in realistic virtual environment},
  author={Hu, Helen H and Gooch, Amy A and Thompson, William B and Smits, Brian E and Rieser, John J and Shirley, Peter},
  booktitle={Proceedings of the conference on Visualization'00},
  pages={179--185},
  year={2000},
  organization={IEEE Computer Society Press}
}



@article{lei13,
  author = { Y. Lei, S. F. Miller },
  title = {Pose estimation and machining efficiency of an endoscopic grinding tool},
  booktitle = { The International Journal of Advanced Manufacturing Technology},
  OPTpages = {1–11},
  year = {2013},
}

@inproceedings{zhesu15a,
  title={Force estimation and slip detection/classification for grip control using a biomimetic tactile sensor},
  author={Su, Zhe and Hausman, Karol and Chebotar, Yevgen and Molchanov, Artem and Loeb, Gerald E and Sukhatme, Gaurav S and Schaal, Stefan},
  booktitle={Humanoid Robots (Humanoids), 2015 IEEE-RAS 15th International Conference on},
  pages={297--303},
  year={2015},
  organization={IEEE}
}

@inproceedings{karayiannidis14a,
  title={Online contact point estimation for uncalibrated tool use},
  author={Karayiannidis, Yiannis and Smith, Christian and Vina, Francisco E and Kragic, Danica},
  booktitle={2014 IEEE Int. Conf. on Robotics and Automation (ICRA)},
  pages={2488--2494},
  year={2014},
  organization={IEEE}
}

% --- Tactile object recognition
@article{pezzementiPRH11,
  author = {Pezzementi, Zachary A. and Plaku, Erion and Reyda, Caitlin and Hager, Gregory D.},
  ee = {http://dx.doi.org/10.1109/TRO.2011.2125350},
  interhash = {c0196a15d4ad39d7cb5977285bcc6ab1},
  intrahash = {4e16cab1ff0f9827de056e79f5f94061},
  journal = {IEEE Transactions on Robotics},
  keywords = {dblp},
  number = 3,
  pages = {473-487},
  timestamp = {2011-08-13T11:31:47.000+0200},
  title = {Tactile-Object Recognition From Appearance Information.},
  volume = 27,
  year = 2011
}
%   url = {http://dblp.uni-trier.de/db/journals/trob/trob27.html#PezzementiPRH11},


% ---- Contact estimation applications
@inproceedings{li15,
  author = {Li, Shuai and Lyu, Siwei and Trinkle, Jeff and Burgard, Wolfram},
  booktitle = {IROS},
  ee = {http://dx.doi.org/10.1109/IROS.2015.7354089},
  interhash = {770ca6dc9c4216bcf2b6640e7af54f12},
  intrahash = {ab032864cb8f16fd11b1c634628e4f2e},
  isbn = {978-1-4799-9994-1},
  keywords = {dblp},
  pages = {5059-5064},
  publisher = {IEEE},
  timestamp = {2016-01-05T11:45:26.000+0100},
  title = {A comparative study of contact models for contact-aware state estimation.},
  year = 2015
}
%   url = {http://dblp.uni-trier.de/db/conf/iros/iros2015.html#LiLTB15},



% ---- Tactile: other
@article{johansson09,
  title={Coding and use of tactile signals from the fingertips in object manipulation tasks},
  author={Johansson, Roland S and Flanagan, J Randall},
  journal={Nature Reviews Neuroscience},
  volume={10},
  number={5},
  pages={345--359},
  year={2009},
  publisher={Nature Publishing Group}
}

@inproceedings{ciobanu14,
  title={Point of contact location and normal force estimation using biomimetical tactile sensors},
  author={Ciobanu, Vlad and Popescu, Decebal and Petrescu, Adrian},
  booktitle={Complex, Intelligent and Software Intensive Systems (CISIS), 2014 Eighth International Conference on},
  pages={373--378},
  year={2014},
  organization={IEEE}
}



@inproceedings{pezzementi11,
  author = {Pezzementi, Zachary A. and Reyda, Caitlin and Hager, Gregory D.},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2011.5980363},
  interhash = {7381fcf75c33de2a281135a88e695e78},
  intrahash = {9b65b190404310a32df428785ff0d036},
  keywords = {dblp},
  pages = {5942-5948},
  publisher = {IEEE},
  timestamp = {2011-08-18T11:33:17.000+0200},
  title = {Object mapping, recognition, and localization from tactile geometry.},
  year = 2011
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2011.html#PezzementiRH11},



@inproceedings{LiPYPRSA14,
  author = {Li, Rui and Jr., Robert Platt and Yuan, Wenzhen and ten Pas, Andreas and Roscup, Nathan and Srinivasan, Mandayam A. and Adelson, Edward H.},
  booktitle = {IROS},
  ee = {http://dx.doi.org/10.1109/IROS.2014.6943123},
  interhash = {cdf9ababe1b85e2eaada9a09881efaae},
  intrahash = {729b710ff275f62a0af654c1cafd61f5},
  keywords = {dblp},
  pages = {3988-3993},
  publisher = {IEEE},
  timestamp = {2015-06-19T14:05:07.000+0200},
  title = {Localization and manipulation of small parts using GelSight tactile sensing.},
  year = 2014
}
%   url = {http://dblp.uni-trier.de/db/conf/iros/iros2014.html#LiPYPRSA14},



@inproceedings{petrovskaya06,
  author = {Petrovskaya, Anna and Khatib, Oussama and Thrun, Sebastian and Ng, Andrew Y.},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ROBOT.2006.1641793},
  interhash = {016f6e40e07831f2a8964a8313cd028c},
  intrahash = {dc1cdf310432c873deec96873aa89743},
  keywords = {dblp},
  pages = {707-714},
  publisher = {IEEE},
  timestamp = {2013-02-21T11:59:29.000+0100},
  title = {Bayesian Estimation for Autonomous Object Manipulation based on Tactile Sensors.},
  year = 2006
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2006.html#PetrovskayaKTN06},


@article{lwpr,
  author = {Vijayakumar, S. and D'Souza, A. and Schaal, S.},
  ee = {http://dx.doi.org/10.1162/089976605774320557},
  interhash = {b659d1187464ca7b8b4d83e6bb59ed3b},
  intrahash = {f556d8cd47d1e3bf2ffc3ca02f49ed77},
  journal = {Neural Computation},
  keywords = {dblp},
  number = 12,
  pages = {2602-2634},
  timestamp = {2011-11-18T11:33:40.000+0100},
  title = {Incremental Online Learning in High Dimensions.},
  volume = 17,
  year = 2005
}

@article{moller93,
  author = {Moller, M. F.},
  groups = {public},
  interhash = {e9ce8863f8066e72b713e8445d76625c},
  intrahash = {43f12f7a9679517454deab4c544d1fe9},
  journal = {Neural Networks},
  keywords = {},
  number = 4,
  pages = {525-533},
  timestamp = {2012-08-18T20:41:53.000+0200},
  title = {{A} Scaled Conjugate Gradient Algorithm for Fast Supervised Learning},
  username = {dalbem},
  volume = 6,
  year = 1993
}

@ARTICLE{marquardt, 
author={Hagan, M.T. and Menhaj, M.B.}, 
journal={Neural Networks, IEEE Transactions on}, 
title={Training feedforward networks with the Marquardt algorithm}, 
year={1994}, 
month={Nov}, 
volume={5}, 
number={6}, 
pages={989-993}, 
ISSN={1045-9227}}

@article{su2012use,
  title={Use of tactile feedback to control exploratory movements to characterize object compliance},
  author={Su, Z. and Fishel, J.A. and Yamamoto, T. and Loeb, G.E.},
  journal={Frontiers in neurorobotics},
  volume={6},
  year={2012},
  publisher={Frontiers Media SA}  
}

@techreport{dogar10,
     title = {{Proprioceptive Localization for Mobile Manipulators}},
     author = {Dogar, M Hemrajani, V Leeds, D Kane, B Srinivasa, S},
     year = {2010},
     institution = {Carnegie Mellon University, Robotics Institute},
     month = {02}
}

@inproceedings{fox12,
  author = {Fox, Charles W. and Evans, Mathew H. and Pearson, Martin J. and Prescott, Tony J.},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2012.6224813},
  interhash = {37c59909036aeaee1752d833dd2e5ab8},
  intrahash = {743b74410791fb24e82596c87b2b6a58},
  isbn = {978-1-4673-1403-9},
  keywords = {dblp},
  pages = {4925-4930},
  publisher = {IEEE},
  timestamp = {2012-07-20T11:35:16.000+0200},
  title = {Tactile SLAM with a biomimetic whiskered robot.},
  year = 2012
}
%   url = {http://dblp.uni-trier.de/db/conf/icra/icra2012.html#FoxEPP12},



% Tactile: human studies papers

@ARTICLE{birznieks98, 
author={Birznieks, I. and Burstedt, M.K.O. and  Edin, B.B. and Johansson, R.S. }, 
journal={Journal of Neurophysiology}, 
title={Mechanisms for force adjustments to unpredictable frictional changes
at individual digits during two-fingered manipulation}, 
year={1998}, 
volume={80}, 
number={4}, 
pages={1989-2002} 
}


@ARTICLE{johanson09, 
author={Johansson, R. S.  and Flanagan, J. R. }, 
journal={Nat. Rev. Neurosci.}, 
title={Coding and use of tactile signals from the fingertips in object manipulation tasks}, 
year={2009}, 
volume={10}, 
pages={345-359} 
}

@ARTICLE{srinivasan90, 
author={Srinivasan, M.A.  and Whitehouse, J.M.  and LaMotte, R.H.  }, 
journal={Journal of Neurophysiology}, 
title={Tactile detection of slip: Surface microgeometry and peripheral neural codes}, 
year={1990}, 
volume={63}, 
pages={1323–1332} 
}

% Tactile grasp control

@inproceedings{maria15,
  author = {De Maria, G. and Falco, P. and Natale, C. and Pirozzi, S.},
  title = {Integrated Force/Tactile Sensing: The Enabling Technology for Slipping Detection and Avoidance},
  booktitle = {IEEE Int. Conf. on Robotics and Automation (ICRA)},
  OPTpages = {26-30},
  year = {2015},
  OPTaddress = {Seattle, Washington},
  OPTmonth = {May},
}

@ARTICLE{romano11, 
author={Romano, J.M. and Hsiao, K. and  Niemeyer, G. and Chitta, S. and  Kuchenbecker, K.J.  }, 
journal={IEEE TRANSACTIONS ON ROBOTICS}, 
title={Human-Inspired Robotic Grasp Control With Tactile Sensing}, 
year={2011}, 
month={Dec},
volume={27}, 
pages={1067-1079} 
}

% Slip detection and slip-based control papers
@inproceedings{mariaNP13,
  author = {Maria, Giuseppe De and Natale, Ciro and Pirozzi, Salvatore},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ICRA.2013.6631070},
  interhash = {7aae33ae8683d8db7283eb5b15df6585},
  intrahash = {50c2bd9e3c9b8e6b377483cffc643609},
  keywords = {dblp},
  pages = {3523-3528},
  publisher = {IEEE},
  timestamp = {2013-10-23T11:35:10.000+0200},
  title = {Slipping control through tactile sensing feedback.},
  year = {2013}
}



@INPROCEEDINGS{heynemanC13, 
author={Heyneman, B. and Cutkosky, M.R.}, 
booktitle={IEEE  Int. Conf. on Intelligent Robots and Systems (IROS)}, 
title={Slip interface classification through tactile signal coherence}, 
year={2013}, 
pages={801-808}, 
ISSN={2153-0858},}

@inproceedings{gunji08,
  author = {Gunji, Daisuke and Mizoguchi, Yoshitomo and Teshigawara, Seiichi and Ming, Aiguo and Namiki, Akio and Ishikawaand, Masatoshi and Shimojo, Makoto},
  booktitle = {ICRA},
  date = {2008-11-06},
  description = {dblp},
  ee = {http://dx.doi.org/10.1109/ROBOT.2008.4543605},
  interhash = {146eddc0fe817d1a78c65a8e7380f826},
  intrahash = {2e8f83e7690fce6fd9f7fb51c2a5ce6b},
  keywords = {dblp},
  pages = {2605-2610},
  publisher = {IEEE},
  timestamp = {2008-11-07T11:35:22.000+0100},
  title = {Grasping force control of multi-fingered robot hand based on slip detection using tactile sensor.},
  year = 2008
}

@article{vatani13,
year={2013},
journal={Sensors and Actuators A: Physical},
volume={195},
title={Force and slip detection with direct-write compliant tactile sensors using multi-walled carbon nanotube/polymer composites},
author={Vatani, M.  and Engeberg, E. D. and Choi, J.-W. },
pages={90-97},
language={English}
}

@article{mariaRAS13,
year={2013},
journal={Robotics and Autonomous Systems},
volume={61},
title={Tactile data modeling and interpretation for stable grasping and manipulation},
author={De Maria, G.  and Natale, C.  and Pirozzi, S. },
pages={1008–1020},
language={English}
}


@article{cavallo14,
year={2014},
journal={Mechatronics},
volume={24},
title={Slipping detection and avoidance based on Kalman filter},
author={Cavallo, A. and De Maria, G.  and Natale, C.  and Pirozzi, S. },
pages={89–2499},
language={English}
}


@inproceedings{engeberg11,
  author = {Engeberg, Erik D. and Meek, Sanford G.},
  booktitle = {IROS},
  ee = {http://dx.doi.org/10.1109/IROS.2011.6094500},
  interhash = {64426156ed47f6bf5b9de5ce50e98ff3},
  intrahash = {65d01989d33c639a2b8765a768100b44},
  isbn = {978-1-61284-454-1},
  keywords = {dblp},
  pages = {4174-4179},
  publisher = {IEEE},
  timestamp = {2011-12-16T11:43:00.000+0100},
  title = {Adaptive sliding mode control of grasped object slip for prosthetic hands.},
  year = 2011
}

@article{melchiorri00,
year={2000},
journal={IEEE/ASME Trans. on Mechatronics},
volume={5},
number={3}, 
title={Slip detection and control using tactile and force sensors},
author={Melchiorri, C.},
pages={235–242},
language={English}
}

@inproceedings{schoepfer10,
  author = {Schoepfer, M. and Schuermann, C. and Pardowitz, M. and Ritter H.},
  title = {Using a Piezo-Resistive Tactile Sensor for Detection of Incipient Slippage},
  booktitle = {IEEE Int. Symp. on Robotics},
  OPTpages = {14–20},
  year = 2010,
  OPTaddress = {Berlin},
}

@article{song14,
  author = {Song, Xiaojing and Liu, Hongbin and Althoefer, Kaspar and Nanayakkara, Thrishantha and Seneviratne, Lakmal D.},
  ee = {http://dx.doi.org/10.1109/TRO.2013.2279630},
  interhash = {ac1b8a520b0425b177a2263494e13fdc},
  intrahash = {0df6005601fae5ee7ff314a615c749f2},
  journal = {IEEE Transactions on Robotics},
  keywords = {dblp},
  number = 1,
  pages = {203-219},
  timestamp = {2015-06-18T09:24:17.000+0200},
  title = {Efficient Break-Away Friction Ratio and Slip Prediction Based on Haptic Surface Exploration.},
  volume = 30,
  year = 2014
}

% Sensors

%BioTac
@article{wettels08,
  title={Biomimetic tactile sensor array},
  author={Wettels, Nicholas and Santos, Veronica J and Johansson, Roland S and Loeb, Gerald E},
  journal={Advanced Robotics},
  volume={22},
  number={8},
  pages={829--849},
  year={2008},
  publisher={Taylor \& Francis}
}



@inproceedings{maria12,
  author = {De Maria, G.  and Natale, C.  and Pirozzi, S. },
  title = {Tactile sensor for human-like manipulation},
  booktitle = {IEEE Int. Conf. on Biomedical Robotics and Biomechatronics},
  OPTpages = {1686–1691},
  year = {2012},
  OPTaddress = {Rome},
}

@inproceedings{schmitz08,
  author = {Schmitz, Alexander and Maggiali, Marco and Randazzo, Marco and Natale, Lorenzo and Metta, Giorgio},
  booktitle = {Humanoids},
  ee = {http://dx.doi.org/10.1109/ICHR.2008.4755988},
  interhash = {b10c2d810d99093712460019aa08f9cc},
  intrahash = {6a3370453e29d564e3c1bff477edf8c0},
  isbn = {978-1-4244-2821-2},
  keywords = {dblp},
  pages = {423-428},
  publisher = {IEEE},
  timestamp = {2012-05-22T11:36:49.000+0200},
  title = {A prototype fingertip with high spatial resolution pressure sensing for the robot iCub.},
  year = {2008}
}

@inproceedings{martin04,
  author = {Martin, Toby B. and Ambrose, Robert O. and Diftler, Myron A. and Jr., Robert Platt and Butzer, Melissa},
  booktitle = {ICRA},
  date = {2007-11-02},
  description = {dblp},
  ee = {http://dx.doi.org/10.1109/ROBOT.2004.1308071},
  interhash = {df441e0a83eecab7130ca73f9f30ace3},
  intrahash = {84335242c4918b8c3c50e628eb7f9db9},
  keywords = {dblp},
  pages = {1713-1718},
  publisher = {IEEE},
  timestamp = {2007-11-03T10:36:06.000+0100},
  title = {Tactile Gloves for Autonomous Grasping with the NASA/DARPA Robonaut.},
  year = 2004
}


% Tactile control: other 
@article{yussof08,
  author = {Yussof, Hanafiah B. and Ohka, Masahiro and Suzuki, Hirofumi and Morisawa, Nobuyuki and Takata, Jumpei},
  date = {2009-11-14},
  description = {dblp},
  ee = {http://www.engineeringletters.com/issues_v16/issue_2/EL_16_2_09.pdf},
  interhash = {49e56f6ff41fbafbd1a009787514d0a9},
  intrahash = {0ebe78e965f0d5c216dee246fe1a3079},
  journal = {Engineering Letters},
  keywords = {dblp},
  number = 2,
  pages = {236-247},
  timestamp = {2009-11-17T11:35:12.000+0100},
  title = {Tactile Sensing-Based Control Architecture in Multi-Fingered Arm for Object Manipulation.},
  volume = 16,
  year = 2008
}

@inproceedings{takahashi08,
  author = {Takahashi, Taro and Tsuboi, Toshimitsu and Kishida, Takeo and Kawanami, Yasunori and Shimizu, Satoru and Iribe, Masatsugu and Fukushima, Tetsuharu and Fujita, Masahiro},
  booktitle = {ICRA},
  date = {2008-11-06},
  description = {dblp},
  ee = {http://dx.doi.org/10.1109/ROBOT.2008.4543219},
  interhash = {3b2beca5e7a0cdbcc86d816ab531bfd4},
  intrahash = {7e66f8418019e491cff31c0d2c3738fa},
  keywords = {dblp},
  pages = {264-271},
  publisher = {IEEE},
  timestamp = {2008-11-07T11:35:24.000+0100},
  title = {Adaptive grasping by multi fingered hand with tactile sensor based on robust force and position control.},
  year = 2008
}





% Neural networks

@article{earlystopping,
year={2007},
issn={0176-4276},
journal={Constructive Approximation},
volume={26},
number={2},
title={On Early Stopping in Gradient Descent Learning},
publisher={Springer-Verlag},
author={Yao, Y. and Rosasco, L. and Caponnetto, A.},
pages={289-315},
language={English}
}


% Learning from tactile information

@inproceedings{Chebotar14,
  author = {Chebotar, Yevgen and Kroemer, Oliver and Peters, Jan},
  booktitle = {IROS},
  ee = {http://dx.doi.org/10.1109/IROS.2014.6943031},
  interhash = {e4b0ac0eb41d4478be453da5b70851a7},
  intrahash = {e9a563d43be64f3097dff321719e6c5d},
  keywords = {dblp},
  pages = {3368-3375},
  publisher = {IEEE},
  timestamp = {2015-06-19T14:05:07.000+0200},
  title = {Learning robot tactile sensing for object manipulation.},
  year = 2014
}


@article{kinoshita1997tangential,
  title={Tangential torque effects on the control of grip forces when holding objects with a precision grip},
  author={Kinoshita, H. and B{\"a}ckstr{\"o}m, L. and Flanagan, J.R. and Johansson, R.S.},
  journal={Journal of Neurophysiology},
  volume={78},
  number={3},
  pages={1619--1630},
  year={1997},
  publisher={Am Physiological Soc}
}

@inproceedings{dahiya2009better,
  title={Better manipulation with human inspired tactile sensing},
  author={Dahiya, Ravinder S and Gori, Monica and Metta, Giorgio and Sandini, Giulio},
  booktitle={RSS 2009 workshop on Understanding the Human Hand for Advancing Robotic Manipulation. RSS},
  pages={1--2},
  year={2009}
}

@inproceedings{erhan2014scalable,
  title={Scalable object detection using deep neural networks},
  author={Erhan, D. and Szegedy, C. and Toshev, A. and Anguelov, D.},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2014 IEEE Conference on},
  pages={2155--2162},
  year={2014},
  organization={IEEE}
}

@article{johansson,
  abstract = {During object manipulation tasks, the brain selects and implements action-phase controllers that use sensory predictions and afferent signals to tailor motor output to the physical properties of the objects involved. Analysis of signals in tactile afferent neurons and central processes in humans reveals how contact events are encoded and used to monitor and update task performance.},
  added-at = {2009-05-19T18:00:18.000+0200},
  author = {Johansson, R.S. and Flanagan, R.J.},
  citeulike-article-id = {4372709},
  description = {CiteULike: Everyone's library},
  interhash = {a9a13958d21babd9721824a865db9731},
  intrahash = {1ddc5f9f90e4c4a7901305068b78f134},
  journal = {Nature Reviews Neuroscience},
  keywords = {imported},
  month = {April},
  number = 5,
  pages = {345--359},
  posted-at = {2009-05-19 14:38:00},
  priority = {2},
  publisher = {Nature Publishing Group},
  timestamp = {2009-05-19T18:03:27.000+0200},
  title = {Coding and use of tactile signals from the fingertips in object manipulation tasks},
  volume = 10,
  year = 2009
}

@incollection{biotacmulti,
year={2014},
booktitle={The Human Hand as an Inspiration for Robot Hand Development},
volume={95},
series={Springer Tracts in Advanced Robotics},
title={Multimodal Tactile Sensor},
publisher={Springer},
keywords={Force and tactile sensing; Biomimetics; Dexterous manipulation; Thermal sensing; Texture},
author={Wettels, N. and Fishel, J.A. and Loeb, G.E.},
pages={405-429},
language={English}
}

@article{wettels2009grip,
  title={Grip control using biomimetic tactile sensing systems},
  author={Wettels, N. and Parnandi, A.R. and Moon, J. and Loeb, G.E. and Sukhatme, G.S.},
  journal={Mechatronics, IEEE/ASME Transactions on},
  volume={14},
  number={6},
  pages={718--723},
  year={2009},
  publisher={IEEE}
}

@inproceedings{WettelsL11,
  added-at = {2012-04-18T00:00:00.000+0200},
  author = {Wettels, N. and Loeb, G.E.},
  booktitle = {ROBIO},
  ee = {http://dx.doi.org/10.1109/ROBIO.2011.6181676},
  interhash = {39399587989e536e8c534ba54f43f47b},
  intrahash = {2019703d42a3d7b06d923dd33f338dc8},
  keywords = {dblp},
  pages = {2471-2478},
  publisher = {IEEE},
  timestamp = {2012-04-19T11:44:37.000+0200},
  title = {Haptic feature extraction from a biomimetic tactile sensor: Force, contact location and curvature.},
  year = 2011
}


% -------------------------------------------
% Machine learning algorithms

@inproceedings{ester96,
  title={A density-based algorithm for discovering clusters in large spatial databases with noise.},
  author={Ester, Martin and Kriegel, Hans-Peter and Sander, J{\"o}rg and Xu, Xiaowei and others},
  booktitle={Kdd},
  volume={96},
  number={34},
  pages={226--231},
  year={1996}
}

@article{selesnickB98,
  added-at = {2012-01-29T00:00:00.000+0100},
  author = {Selesnick, Ivan W. and Burrus, C. Sidney},
  ee = {http://dx.doi.org/10.1109/78.678493},
  interhash = {118c9c985cd2d22147ba5b3bc76d3342},
  intrahash = {8f864cf31b81921f91895ae9a16bd393},
  journal = {IEEE Transactions on Signal Processing},
  keywords = {dblp},
  number = 6,
  pages = {1688-1694},
  timestamp = {2012-01-31T11:33:28.000+0100},
  title = {Generalized digital Butterworth filter design.},
  volume = 46,
  year = 1998
}
%   url = {http://dblp.uni-trier.de/db/journals/tsp/tsp46.html#SelesnickB98},


@article{srivastavaHKSS14,
  title={Dropout: a simple way to prevent neural networks from overfitting.},
  author={Srivastava, Nitish and Hinton, Geoffrey E and Krizhevsky, Alex and Sutskever, Ilya and Salakhutdinov, Ruslan},
  journal={Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={1929--1958},
  year={2014}
}

@inproceedings{krizhevsky12,
  added-at = {2015-11-20T13:12:04.000+0100},
  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle = {Advances in neural information processing systems},
  interhash = {74bbb5dea5afb1b088bd10e317f1f0d2},
  intrahash = {784f6d0ddce5f78d5d2105a1781cecc2},
  keywords = {classification image imagenet thema:deepwalk},
  pages = {1097--1105},
  timestamp = {2015-11-20T13:12:04.000+0100},
  title = {Imagenet classification with deep convolutional neural networks},
  year = 2012
}


@article{simonyan14a,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@article{kaneko1994contact,
  title={Contact point detection for grasping an unknown object using self-posture changeability},
  author={Kaneko, Makoto and Tanie, Kazuo},
  journal={IEEE Transactions on Robotics and Automation},
  volume={10},
  number={3},
  pages={355--367},
  year={1994},
  publisher={IEEE}
}

@article{domingos12,
  added-at = {2015-05-07T00:00:00.000+0200},
  author = {Domingos, Pedro M.},
  ee = {http://doi.acm.org/10.1145/2347736.2347755},
  interhash = {28f49d94d3029e886460cde63094e482},
  intrahash = {5ef0b7eda54e28c0f14eabc15925aecf},
  journal = {Commun. ACM},
  keywords = {dblp},
  number = 10,
  pages = {78-87},
  timestamp = {2015-06-17T23:51:59.000+0200},
  title = {A few useful things to know about machine learning.},
  volume = 55,
  year = 2012
}

@inproceedings{chebotar2014learning,
  title={Learning robot tactile sensing for object manipulation},
  author={Chebotar, Yevgen and Kroemer, Oliver and Peters, Jan},
  booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={3368--3375},
  year={2014},
  organization={IEEE}
}

@inproceedings{li2014localization,
  title={Localization and manipulation of small parts using gelsight tactile sensing},
  author={Li, Rui and Platt, Robert and Yuan, Wenzhen and ten Pas, Andreas and Roscup, Nathan and Srinivasan, Mandayam A and Adelson, Edward},
  booktitle={2014 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={3988--3993},
  year={2014},
  organization={IEEE}
}

@inproceedings{su2016tilt,
  title={Surface Tilt Perception with a Biomimetic Tactile Sensor},
  author={Su, Zhe and Schaal, Stefan and Loeb, Gerald E},
  booktitle={ 2016 6th IEEE RAS \& EMBS international conference on biomedical robotics and biomechatronics (BioRob)},
  year={2016 (Accepted)},
  organization={IEEE}
}

@inproceedings{corcoran2010measurement,
  title={A measurement model for tracking hand-object state during dexterous manipulation},
  author={Corcoran, Craig and Platt, Robert},
  booktitle={Robotics and Automation (ICRA), 2010 IEEE International Conference on},
  pages={4302--4308},
  year={2010},
  organization={IEEE}
}

@article{schmidhuber2015deep,
  title={Deep learning in neural networks: An overview},
  author={Schmidhuber, J{\"u}rgen},
  journal={Neural Networks},
  volume={61},
  pages={85--117},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{sharif2014cnn,
  title={CNN features off-the-shelf: an astounding baseline for recognition},
  author={Sharif Razavian, Ali and Azizpour, Hossein and Sullivan, Josephine and Carlsson, Stefan},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition Workshops},
  pages={806--813},
  year={2014}
}

@article{williams2006gaussian,
  title={Gaussian processes for machine learning},
  author={Williams, Christopher KI and Rasmussen, Carl Edward},
  journal={the MIT Press},
  volume={2},
  number={3},
  pages={4},
  year={2006}
}

@inproceedings{su2016sensorimotorprimitive,
  title={Learning to Switch between SensorimotorPrimitives using Multimodal Haptic Signals},
  author={Su, Zhe and Kroemer, Oliver and Loeb, Gerald E and Sukhatme, Gaurav S. and Schaal, Stefan},
  booktitle={International Conference on Simulation of Adaptive Behavior (SAB)},
  year={2016 (Accepted)},
  organization={Springer}
}

@inproceedings{Chebotar2016Regrasping, 
author={Chebotar, Yevgen and Hausman, Karol and Su, Zhe and Sukhatme, Gaurav S. and Schaal, Stefan}, 
booktitle={IEEE  Int. Conf. on Intelligent Robots and Systems (IROS)}, 
title={Self-Supervised Regrasping Using Spatio-Temporal Tactile Features and Reinforcement Learning}, 
year={2016 (Accepted)}, 
organization={IEEE}
}

@article{Kroemer_TRo_2011,
  author ={Kroemer, O. and  Lampert, C.H. and  Peters, J.},
  year ={2011},
  title ={Learning Dynamic Tactile Sensing with Robust Vision-based Training},
  journal ={IEEE Transactions on Robotics (T-Ro)},
  number ={3},
  pages ={545-557}
}

@article{kearns02,
  author    = {Michael J. Kearns and
               Yishay Mansour and
               Andrew Y. Ng},
  title     = {A Sparse Sampling Algorithm for Near-Optimal Planning in Large Markov
               Decision Processes},
  journal   = {Machine Learning},
  volume    = {49},
  number    = {2-3},
  pages     = {193--208},
  year      = {2002}
}


% --- OTHER -------------------------------------------------------------------------

@misc{gym,
        Author = {Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
        Title = {OpenAI Gym},
        Year = {2016},
        Eprint = {arXiv:1606.01540},
}
